Selective Forgetting of Deep Networks at a Finer Level than Samples

Selective forgetting or removing information from deep neural networks (DNNs) is essential for continual learning and is challenging in controlling the DNNs. Such forgetting is crucial also in a practical sense since the deployed DNNs may be trained on the data with outliers, poisoned by attackers, or with leaked/sensitive information. In this paper, we formulate selective forgetting for classification tasks at a finer level than the samples' level. We specify the finer level based on four datasets distinguished by two conditions: whether they contain information to be forgotten and whether they are available for the forgetting procedure. Additionally, we reveal the need for such formulation with the datasets by showing concrete and practical situations. Moreover, we introduce the forgetting procedure as an optimization problem on three criteria; the forgetting, the correction, and the remembering term. Experimental results show that the proposed methods can make the model forget to use specific information for classification. Notably, in specific cases, our methods improved the model's accuracy on the datasets, which contains information to be forgotten but is unavailable in the forgetting procedure. Such data are unexpectedly found and misclassified in actual situations.

==> settings.tex <==
\section{Settings}
\subsection{Constraints}
%% 実験ではこのconstraintに注目します：上のtableのなかで必要性が示されているから! 
%% 


\subsection{Targets for selective forgetting}
%% 忘却対象とその確かめる方法の記述。
%% 実験で扱うより抽象度が低いもの (Typical Situation) + 実験時レベル
\com{Concat with targets and situasions}
A brief target of the selective forgetting is a subset of a training dataset. 
An illustrative situation is when a class is no longer needed in a classification problem.
In our experiment, we set the target to be a class of the classification problem of images. 
In addition, we check whether the classification accuracy is low for the class to be forgotten and kept high for the class left behind.

A typical target of the selective forgetting is the decision-making basis of the machine learning model.
An example is the background or style of images in the image classification task.
Another example of the target is an undesired sign, symbol, or code that was included in the training data that was discovered after training. 
In this experiment, we target such backdoor features in the input images in a specified class. 
We confirm that the modified model retains a high classification accuracy for the data without backdoors.

%% q1. 学習データのサブセットを忘れる
%% q2. ある入力データが望まないleakage/backdoor/patternを含んでいるとする.　そのbackdoorを取り除いた入力に対しても正しく分類判断できるように修正する、他のクラスに影響を与えないように。


%%%% 分類実験でのフォーミュレーション
%%  --> t1. あるクラスの学習データのみを用いで、そのクラスの分類精度を下げる、他のクラスに影響を与えないように。 (to q1)
%%  --> t2. あるクラスの学習データにleakage/backdoor/patternを加えて学習されたモデルが、そのクラスのcleanなデータを正しく分類できるようにする.


